Generalizing Roberts' characterization of unit interval graphs

For any natural number $d$, a graph $G$ is a (disjoint) $d$-interval graph if it is the intersection graph of (disjoint) $d$-intervals, the union of $d$ (disjoint) intervals on the real line. Two important subclasses of $d$-interval graphs are unit and balanced $d$-interval graphs (where every interval has unit length or all the intervals associated to a same vertex have the same length, respectively). A celebrated result by Roberts gives a simple characterization of unit interval graphs being exactly claw-free interval graphs. Here, we study the generalization of this characterization for $d$-interval graphs. In particular, we prove that for any $d \geq 2$, if $G$ is a $K_{1,2d+1}$-free interval graph, then $G$ is a unit $d$-interval graph. However, somehow surprisingly, under the same assumptions, $G$ is not always a \emph{disjoint} unit $d$-interval graph. This implies that the class of disjoint unit $d$-interval graphs is strictly included in the class of unit $d$-interval graphs. Finally, we study the relationships between the classes obtained under disjoint and non-disjoint $d$-intervals in the balanced case and show that the classes of disjoint balanced 2-intervals and balanced 2-intervals coincide, but this is no longer true for $d>2$.

==> Sections/Section7.tex <==
%these are roughly the implications that follow directly

In this section, we highlight the implications of our results in the field of preference modeling and order theory.

\begin{corollary}
Let $X$ be a set of elements and let $T\subseteq X \times X$ be a set of tuples of elements of $X$, where each element appears in at most one tuple. Let $\prec$ be a partial order on the set of tuples $T$ without $1+5$. Then, there exists a semiorder $P$ on the elements of $X$ such that if two tuples $(x_1, x_2)$, $(y_1,y_2)$ are incomparable with respect to $\prec$, then at least one pair $x_i, y_j$, with $i,j\in\{1,2\}$, is incomparable. Furthermore, given the partial order $\prec$, we can construct $P$ in linear time.
%elements are incomparable only if the two tuples they belong to are incomparable, and 
\end{corollary}

\begin{corollary}
Let $X$ be a set of elements and let $f$ be a bi-dimensional preference function. Let $\prec$ be a partial ordering on the preferences of the elements of $X$ without $1+5$. Then, there exists a semiorder $\prec_P$ on the two dimensions of the elements of $X$ such that if two elements are indifferent with respect to $\prec$, then the two elements are indifferent in at least one of their dimensions.
%However, if for every element, one of the dimensions is strictly preferred than the other, such a semiorder does not necessarily exist. 
\end{corollary}




==> Sections/hardness.tex <==
In this section, we prove that even though there is an easy characterization of unit 2-interval graphs which are also interval, the general problem of recognizing unit 2-interval graphs remains \NP-complete, as the problem of recognizing disjoint unit 2-interval graphs, proven recently in \cite{acceptedvirginia}.

\begin{theorem}
    Deciding whether a graph is a unit 2-interval graph is \NP-complete.
\end{theorem}

\begin{proof}
    We use the same reduction as in the proof of \NP-hardness of recognizing disjoint unit 2-interval graphs in \cite{acceptedvirginia}.
    That is, given a formula $\Phi$ satisfying the conditions described, we construct the same graph $G$. The reader can see that one of the directions still holds directly for the non-disjoint case: if the formula is satisfiable and there exists a disjoint unit 2-interval representation, then there also exists a disjoint unit 2-interval representation, as the class of disjoint unit 2-interval graphs is contained in the class of unit 2-interval  graphs.
 On the other hand, to prove the other direction, we simply need to adapt the proof of Claim 6. 
 
 Note that the characterization of colored unit 2-interval graphs in Lemma 5 needs to be slightly modified for the non-disjoint case, as when we split a vertex, now we can have an edge between its two representatives. That is, condition 3 in the definition of a split of a graph needs to be removed, as $f^{-1}(v)$ does not need to be an independent set anymore. 
 
 This has as effect on the proof of Claim 6, where it is shown that no black vertex can be adjacent to two representatives of the same vertex because it would form a $K_{1,3}$. This is no longer true in the non-disjoint case, as there could be an edge between them, and so they would not form an induced $K_{1,3}$. However, the result still follows because if a black vertex is adjacent to two representatives of the same vertex, then there would be an induced net. Let us prove that.

 \begin{claim}
     Suppose that a black vertex is adjacent to two representatives of the same vertex. Then, the constructed graph $G$ cannot be a unit interval graph.
 \end{claim}
 \begin{proof}
Claim 6: it holds that if a black vertex is adjacent to a representative of $x_i^1$ and to a representative of $x_i^2$, these two representatives must be adjacent to each other.

Claim 7: holds completely. When it uses Claim 6, it uses the part that holds.
First case:
----
Then, if one representative of $x_i^N$ is adjacent to both $A_i$ and $B_i$, then we must have one rep of each positive literal each to a different vertex $A_i$ or $B_i$. Furthermore, no two representatives of the same literal vertex can be adjacent to each other, because we create the cycle of length 5 $x_11, A, x_N, B, x_12$. On the other hand, the other representative of $x_i^N$ can either be isolated or adjacent the first representative, and if it is adjacent, it must be a twin.

Claim
If the other representative is adjacent, it must be a twin or intersect only one of $A_i$ or $B_i$ (the one who is not adjacent to the copy of positive literal representatives adjacent to $C_i$.

First, it must be adjacent to at least one $A_i$ or $B_i$ (otherwise $[x_i^N 1, A_i, B_i, x_i^N 2)$. W.l.o.g., suppose that $x_i^1 1$ and $x_i^2 1$ are adjacent to $A_i$ and $C_i$. Then, the other representative of $x_i^N$ can be adjacent to $B_i$ only. On the other hand, if it is adjacent to $A_i$, it must be a twin. First, it must be adjacent to $C_i$, because otherwise there is a net: $C_i, B_i, x_N 1, x_N2, x_22, x_11$. And so to $B_i$ to avoid an induced $K_{1,3}$.

claim.
If the two representatives are adjacent, then there is a net in the constructed graph $G$. 
proof.
If $x_N2$ is only adjacent to $B_i$. Since at least one of $x_N$ is adjacent to a private neighbor. If it is the second representative, we have the net: $B_i, x_N1, x_n2, A_i, x_11$ and the private neighbor.
Otherwise, the net $B,C,x_N1, x_11, x_12$, private neighbor.
If the two representatives are twins, and the second one has a private neighbor, we have the net $C_i, B_i, x_N2, x_11, x_12$ and private neighbor.
If the first one has an external neighbor, we have the net $C_i, B_i, x_N1, x_11, x_12$ and private. 



%(as otherwise there would be an induced $K_{1,3}$ with center $C_i$, because the other representative need to be adjacent to $C_i$ to avoid a $K_{1,3}$ with center $x_N$ and leaves $A_i$. 

-------
2nd case:

If one representative of $x_i^N$ is adjacent to $A_i$ and the other to $B_i$, then at least one representative of $x_i^1$ and $x_i^2$ must be adjacent to both $A_i$ and $B_i$.
The other representatives can be either isolated vertices or be twins of the first representatives (prove the last statement). Actually, we can also have one representative for each, i.e., case in claim 9 which is not possible, and case in claim 11 which is still not possible either.

If at least one positive representative is adjacent to both $A_i$ and $B_i$, the two negative representatives cannot be adjacent, because then there is a cycle with these 3, $A_i$ and $B_i$.
%If two representatives of the same vertex are adjacent, they must be twins. 
They cannot be as in claim 9 or claim 11 in cite. That means that for both positive literals, at least one representative is adjacent to both $A_i$ and $B_i$. 

claim
If the other representatives are not isolated, then they are twins with the first representative.
If wlog x12 is adjacent only to a black vertex, it creates a k13, so it must form a clique with the positive literals that were already adjacent to the black vertex %(and be adjacent to all the black vertices).
If instead it is only adjacent to a positive literal x11 or x21, then it will create a net (for example, C,A, x21, x12,xn1, xn2 if it is adjacent to x21). However, it could be that x12 is adjacent to x22.

claim
If one of the black vertices is adjacent to two representatives of the same positive literal (in this second case), then $G$ is not unit interval.
proof.
Notice that both representatives can't be adjacent to both $A_i$ and $B_i$, because at least one has a private neighbor in $G$, which would create an induced $K_{1,3}$. So assume that both representatives of one positive literal, say x1, are adjacent to $B_i$ (resp, $A_i$). Then there is an induced tent formed by $B, x11, x12, A, XN$ and the private neighbor.


Prove that in case 1 we need the negative one to be free for no nets.
In case 2 we need 
Lemma 8 changes: 
1. ... while for the rest of the literal vertices, all the representatives adjacent to A form a clique, all the representatives adjacent to B form a clique (there can also be isolated ones, but of course, at least one of each must be adjacent): it can be 
2. One representative of $x_i^N$ is adjacent to both $A_i$ and $B_i$, and one representative of each of the positive literal each to a different vertex from $A$ and $B$. The other representative

\begin{comment}
    
 This holds: if a black vertex is adjacent to a representative of $x_i^1$ or $x_i^2$, these two representatives must be adjacent. 
 This holds: either 1) the vertex $f^{-1}(x_i^N)$ is adjacent to $A_i$ and the other to $B_i$. 2) This doesn't hold exactly, because they could be adjacent to both: The two representatives of positive literals adjacent to A are adjacent to each other, and other two adjacent to B. This claim should maybe be: no representative can be adjacent to both B and A. 
 
Suppose first that a black vertex is adjacent to the two representatives of $x_i^N$. 
Suppose that a black vertex is adjacent to two representatives of the same vertex. Then, since it still needs to be adjacent to two other vertices
 net created by : ax, xn1, fx1,x2, b xn2, the outneighbor of fx1 
 \end{comment}
 \end{proof}

 The rest of the proofs hold directly without any changes. Indeed, note that we never make use of forbidden induced subgraphs where there are two representatives of the same vertex.
 
 
\end{proof}

